Only My Model On My Data: A Privacy Preserving Approach Protecting one Model and Deceiving Unauthorized Black-Box Models

Deep neural networks are extensively applied to real-world tasks, such as face recognition and medical image classification, where privacy and data protection are critical. Image data, if not protected, can be exploited to infer personal or contextual information. Existing privacy preservation methods, like encryption, generate perturbed images that are unrecognizable to even humans. Adversarial attack approaches prohibit automated inference even for authorized stakeholders, limiting practical incentives for commercial and widespread adaptation. This pioneering study tackles an unexplored practical privacy preservation use case by generating human-perceivable images that maintain accurate inference by an authorized model while evading other unauthorized black-box models of similar or dissimilar objectives, and addresses the previous research gaps. The datasets employed are ImageNet, for image classification, Celeba-HQ dataset, for identity classification, and AffectNet, for emotion classification. Our results show that the generated images can successfully maintain the accuracy of a protected model and degrade the average accuracy of the unauthorized black-box models to 11.97%, 6.63%, and 55.51% on ImageNet, Celeba-HQ, and AffectNet datasets, respectively.

==> sec/backup.tex <==
\begin{abstract}
Deep neural networks have been widely used in real-world applications for different tasks, wherein privacy and data protection are important, such as face recognition, medical image classification, etc. Image data can be harvested to infer personal information or used to gather contextual information about the subject's surroundings. While existing computer vision methods predominantly focus on generating perturbed 
%encrypting 
images that render them imperceptible to humans, the exploration of generating perceptible images that maintain accurate inference by an authorized protected model while evading other black-box models of similar or dissimilar objectives remains unexplored. This study introduces a novel approach to address this gap, pioneering research in this area by offering comprehensive solutions applicable to diverse tasks, datasets, and models of varying complexities. We validate the efficacy of our proposed solutions across 3 distinct datasets and diverse models.
%~Existing computer vision-based privacy protection methods mainly focus on encrypting the image itself, which makes it imperceptible to humans. The topic of generating perceptible images that can evade black-box target models while protecting an authorized model still remains unexplored. In this work, we propose a novel approach to achieve this goal. 
%that generates perceivable images that can fail the black-box adversaries and keep the performance on our benign model. 
%We validate the effectiveness of our proposed method on four different datasets and across different models. 
The datasets include ImageNet dataset, which is for general image classification, Celeba-HQ dataset, which is for identity classification, and Affectnet, which is for emotion classification.
Our results show that the generated images can maintain the accuracy of a protected model and degrade the average accuracy of the target black-box models to 11.97\%, 6.63\%, and 55.51\% on ImageNet, Celeba-HQ, and Affectnet datasets, respectively.
\end{abstract}
